The GBT Diffuse Ionized Gas Survey (GDIGS): Discrete Sources

The Green Bank Telescope (GBT) Diffuse Ionized Gas Survey (GDIGS) traces ionized gas in the Galactic midplane by observing radio recombination line (RRL) emission from 4-8 GHz. The nominal survey zone is $32.3^{\circ}> {\ell} > -5^{\circ}$, $|b|<0.5^{\circ}$. Here, we analyze GDIGS Hn${\alpha}$ ionized gas emission toward discrete sources. Using GDIGS data, we identify the velocity of 35 H II regions that have multiple detected RRL velocity components. We identify and characterize RRL emission from 88 H II regions that previously lacked measured ionized gas velocities. We also identify and characterize RRL emission from eight locations that appear to be previously-unidentified H II regions and 30 locations of RRL emission that do not appear to be H II regions based on their lack of mid-infrared emission. This latter group may be a compact component of the Galactic Diffuse Ionized Gas (DIG). There are an additional 10 discrete sources that have anomalously high RRL velocities for their locations in the Galactic plane. We compare these objects' RRL data to 13CO, H I and mid-infrared data, and find that these sources do not have the expected 24 ${\mu}$m emission characteristic of H II regions. Based on this comparison we do not think these objects are H II regions, but we are unable to classify them as a known type of object.

==> GDIGS_hii_regions.tex <==
\section{New HII Region Discoveries and Compact DIG Locations\label{sec:discoveries}}
GDIGS data can provide information on the Galactic \hii\ region population by examining RRL emission from \hii\ regions in the {\it WISE} Catalog and by examining locations of RRL emission that were previously uncategorized.  We report here on three uses for the GDIGS data: 1) characterizing RRL emission from {\it WISE} Catalog \hii\ regions not previously detected in RRL emission, 2) identifying new sources of RRL emission, and 3) determining the \hii\ region velocity for \hii\ regions with multiple RRL velocity components reported in the literature.  {\bf For all analyses, we smooth the data to 4.71\,\kms.}
%GDIGS data can also locate regions of RRL emission that are not identified as being \hii\ regions.

%We compute Heliocentric and Galactocentric distances for each RRL detection in the zone $15\degree < \ell < 44\degree$ where kinematic distances are for the most part reliable \citep{anderson09a, wenger18}.  In this zone, each RRL velocity corresponds to two possible heliocentric kinematic distances, known as ``near'' and ``far.'' This dual-distance problem is known as the kinematic distance ambiguity (KDA).  Halfway between the two distances is the tangent point distance, which has the highest velocity along the line of sight.  The Galactocentric distance is unambiguous for each longitude-velocity location.

\subsection{RRL Emission from Discrete HII Regions}
We explore new detections of \hna\ RRL emission from {\it WISE} Catalog sources with the ``group,'' ``candidate,'' and ``radio quiet candidate'' designations.  Due to confusion within the GDIGS beam, the most likely detections are from \hii\ regions that are isolated or are angularly large.

\subsubsection{Group HII Regions}
GDIGS can provide first RRL detections for ``group'' \hii\ regions, which are found in complexes with other known \hii\ regions but have not been detected previously in pointed RRL surveys.  There are $\sim\!150$ {\it WISE} catalog group \hii\ regions in the GDIGS survey zone.  Many of these are confused with brighter nearby \hii\ regions, and so their RRL emission cannot be reliably measured.  There are 39 unconfused group \hii\ regions that we examine for RRL emission.  For each of these, we extract GDIGS \hna\ spectra from a single pixel and fit Gaussian profiles.  

We give the Gaussian fit parameters for the examined group \hii\ regions in Table~\ref{tab:groups}, which lists the source name, the Galactic longitude and latitude, the line intensity, the LSR velocity, the FWHM line width and the rms noise. The errors in Table~\ref{tab:groups} are the 1$\sigma$ uncertainties from the Gaussian fits. We detect RRL emission from 37 of the 39 \hii\ regions.  For the eight spectra best fit with with multiple velocity components, we append to their source names ``a,'' ``b,'' or ``c'' in order of decreasing peak line intensity.  All listed line parameters have a signal-to-noise ratio (SNR) of at least 5, where the SNR
as defined by \citet{lenz92} is
\begin{equation}
    {\rm SNR} = 0.7 \left( \frac{T_{\rm L}}{\rm rms}\right) \left( \frac{\Delta V}{4.71} \right)^{0.5}\,,
\end{equation}
where $T_L$ is the peak line height, rms is the root mean-squared spectral noise, $\Delta V$ is FWHM line width in \kms, and the factor of {\bf 4.71 is the smoothing in \kms}.  We follow this same table format and SNR requirement in all following tables of \hna\ RRL parameters.

\begin{deluxetable*}{lrrrcrcccr}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{\hna\ RRL Parameters from {\bf {\it WISE} Catalog} Group \hii\ Regions}
\tablewidth{0pt}
\tablehead{
\colhead{Source\tablenotemark{$a$}} &
\colhead{\gl} &
\colhead{\gb} & 
\colhead{$T_L$} &
\colhead{$\sigma T_L$} &
\colhead{$V_{LSR}$} &
\colhead{$\sigma V_{LSR}$} &
\colhead{$\Delta V$} &
\colhead{$\sigma \Delta V$} &
\colhead{rms}%& $
%\colhead{Note\tablenotemark{a}}
\\
\colhead{} &
\colhead{($\arcdeg$)} &
\colhead{($\arcdeg$)} &
\colhead{(mK)} &
\colhead{(mK)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(mK)}% &
%\colhead{}
}
\startdata
\input gdigs_groups.tab
\enddata
\label{tab:groups}
\tablenotetext{a}{Source names for HII regions with multiple detected hydrogen RRL components are appended with ``a'' and ``b'' in order of decreasing \hna\ RRL intensity.}
\end{deluxetable*}

The GDIGS RRL velocities of group \hii\ regions indicate that they are for the most part correctly associated with known \hii\ regions.  In Figure~\ref{fig:group}, we plot the measured GDIGS group \hii\ region RRL velocity against the velocity of the known \hii\ region in the same complex.  There is a strong correlation between the two velocities, indicating that the original group associations for this sample were largely correct.  The largest discrepancies are for sources with multiple velocities, where one velocity is likely from the DIG.

\begin{figure}
    \centering
    \includegraphics[width=3in]{glong_vs_vlsr2.pdf}
    \caption{Difference between the measured GDIGS RRL velocity of group \hii\ regions and those of other \hii\ regions in the same complexes, as a function of Galactic longitude.  Group \hii\ regions with two velocities are connected with vertical lines.  The group \hii\ regions have similar velocities as the measured known \hii\ regions, although some of the offsets approach 20\,\kms.}
    \label{fig:group}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{HII Region Candidates}
Within the GDIGS survey range there are $\sim\!500$ {\it WISE} Catalog \hii\ region candidates that have spatially coincident radio continuum and MIR emission.  None of the candidate \hii\ regions have been previously detected in RRL or spectroscopic H$-\alpha$ emission.  {\bf Since the GDIGS area has been searched several times by more
sensitive, pointed RRL surveys \citep[e.g.,][]{anderson11,anderson15a},
any new HII region detections using GDIGS are possible only for
candidate sources that were skipped in previous surveys.}
We examine these $\sim\! 500$ locations find 23 \hii\ region candidates that are unconfused by the RRL emission from other nearby bright \hii\ regions.  We integrate GDIGS \hna\ data over the extent of the sources defined in the {\it WISE} catalog and fit Gaussian components, characterizing the emission from 20 of the 22 candidates.  Eight of the nebulae are best fit with two Gaussian components.  We give their RRL parameters in Table~\ref{tab:candidates}.

\begin{deluxetable*}{lrrrcrcccr}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{\hna\ RRL Parameters from {\bf {\it WISE} Catalog} Candidate \hii\ Regions}
\tablewidth{0pt}
\tablehead{
\colhead{Source\tablenotemark{a}} &
\colhead{\gl} &
\colhead{\gb} & 
\colhead{$T_L$} &
\colhead{$\sigma T_L$} &
\colhead{$V_{LSR}$} &
\colhead{$\sigma V_{LSR}$} &
\colhead{$\Delta V$} &
\colhead{$\sigma \Delta V$} &
\colhead{rms}%& $
%\colhead{Note\tablenotemark{a}}
\\
\colhead{} &
\colhead{($\arcdeg$)} &
\colhead{($\arcdeg$)} &
\colhead{(mK)} &
\colhead{(mK)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(mK)}% &
%\colhead{}
}
\startdata
\input gdigs_candidates2.tab
\enddata
\label{tab:candidates}
\tablenotetext{a}{Source names for HII regions with multiple detected hydrogen RRL components are appended with ``a'' and ``b'' in order of decreasing \hna\ RRL intensity.}
\end{deluxetable*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Radio-quiet HII Region Candidates}
Within the GDIGS survey range there are $\sim\!1200$ {\it WISE} Catalog radio quiet \hii\ region candidates.  These nebulae have the characterisitc MIR morphology of \hii\ regions, but have no detected radio continuum emission in any extant survey.  Given the sensitivity of GDIGS, we therefore do not expect many \hna\ RRL detections.  In the Galactic longitude range $17.5\degree > \ell > -5\degree$, however, the quality of public radio continuum data suitable for identifying \hii\ regions is poor, and GDIGS may be able to identify new Galactic \hii\ regions here.  

To determine if GDIGS detects the emission from any radio-quiet {\it WISE} Catalog sources, we visually inspect the GIDGS \hna\ Moment~0 data (Figure~\ref{fig:coverage}) for isolated emission of a morphology complementary to that of the MIR emission.  We measure RRL emission from 15 {\it WISE} Catalog radio quiet \hii\ region candidates by integrating GDIGS \hna\ data over the extent of the sources defined in the {\it WISE} catalog.  All but one of these is in the zone $17.5\degree > \ell > -5\degree$.
Five of these nebulae are best fit with two Gaussian components, and one with three Gaussian components.  We give their \hna\ RRL parameters in Table~\ref{tab:rq_candidates}.

\begin{deluxetable*}{lrrrcrcccr}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{\hna\ RRL Parameters from {\bf {\it WISE} Catalog} Radio-quiet \hii\ Region Candidates}
\tablewidth{0pt}
\tablehead{
\colhead{Source\tablenotemark{a}} &
\colhead{\gl} &
\colhead{\gb} & 
\colhead{$T_L$} &
\colhead{$\sigma T_L$} &
\colhead{$V_{LSR}$} &
\colhead{$\sigma V_{LSR}$} &
\colhead{$\Delta V$} &
\colhead{$\sigma \Delta V$} &
\colhead{rms}%& $
%\colhead{Note\tablenotemark{a}}
\\
\colhead{} &
\colhead{($\arcdeg$)} &
\colhead{($\arcdeg$)} &
\colhead{(mK)} &
\colhead{(mK)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(mK)}% &
%\colhead{}
}
\startdata
\input gdigs_candidatesrq2.tab
\enddata
\label{tab:rq_candidates}
\tablenotetext{a}{Source names for HII regions with multiple detected hydrogen RRL components are appended with ``a,'' ``b,'' and ``c'' in order of decreasing \hna\ RRL intensity.}
\end{deluxetable*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{New RRL Discoveries}
GDIGS detects some RRL emission that is not smoothly distributed, and not associated with \hii\ regions in the {\it WISE} Catalog.  If the locations of this RRL emission coincide with MIR morphology characteristic of \hii\ regions, we categorize them as newly-disovered \hii\ regions; if not, we characterize them as discrete DIG locations.  {\bf Although all \hii\ regions should be included in the {\it WISE} Catalog,  the GDIGS data allow us to separate complicated regions of the ISM into discrete \hii\ regions.}

\subsubsection{New HII Regions}
There are six locations of GDIGS RRL emission that we believe to be from new Galactic \hii\ regions not included in the {\it WISE} Catalog.  Each of these locations has spatially coincident GDIGS \hna\ and MIR emission.  They were likely missed in the {\it WISE} Catalog because their MIR emission is faint or confused with that of other nearby regions.  We measure RRL emission from these new \hii\ regions by integrating GDIGS \hna\ data over their extents defined using the GDIGS Moment~0 data.  
Four of these nebulae are best fit with two Gaussian components, and one with three Gaussian components.  
We characterize the \hna\ GDIGS emission from these locations in Table~\ref{tab:new}.

\begin{deluxetable*}{lrrrrcrcccr}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{\hna\ RRL Parameters from New \hii\ Regions}
\tablewidth{0pt}
\tablehead{
\colhead{Source\tablenotemark{a}} &
\colhead{\gl} &
\colhead{\gb} & 
\colhead{Radius} &
\colhead{$T_L$} &
\colhead{$\sigma T_L$} &
\colhead{$V_{LSR}$} &
\colhead{$\sigma V_{LSR}$} &
\colhead{$\Delta V$} &
\colhead{$\sigma \Delta V$} &
\colhead{rms}%& $
%\colhead{Note\tablenotemark{a}}
\\
\colhead{} &
\colhead{($\arcdeg$)} &
\colhead{($\arcdeg$)} &
\colhead{(arcmin.)} & 
\colhead{(mK)} &
\colhead{(mK)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(mK)}% &
%\colhead{}
}
\startdata
\input gdigs_newregions2.tab
\enddata
\label{tab:new}
\tablenotetext{a}{Source names for HII regions with multiple detected hydrogen RRL components are appended with ``a'' and ``b'' in order of decreasing \hna\ RRL intensity.}
\end{deluxetable*}

\subsubsection{Locations of Compact DIG Emission}
There are additionally 32 locations of {\bf discrete} GDIGS \hna\ emission identifiable in the Moment~0 maps that, due to a lack of spatially coincident MIR emission, we do not believe to be discrete \hii\ regions.  {\bf These locations have sizes of approximately the GDIGS \hna\ beam.}  Without high-resolution data, we cannot conclusively determine their origin, and here only characterize their \hna\ emission properties.
%The locations are all near to known \hii\ regions and could be the result of photons escaping from those regions.  Their relatively high emission measures indicates that they have high electron densities or long path lengths.  The lack of MIR emission distinguishes these regions from those of known \hii\ regions.
We measure RRL emission from these locations by integrating GDIGS \hna\ data over their extents defined visually using the GDIGS Moment~0 data.  Of the 32 locations, we detect RRL emission from 26; the other six locations are too faint to accurately characterize.
Six of these nebulae are best fit with two Gaussian components.  
We characterize the \hna\ GDIGS emission from these locations in Table~\ref{tab:new_dig}. 

\begin{deluxetable*}{lrrrrcrcccr}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{\hna\ RRL Parameters from Discrete DIG Locations}
\tablewidth{0pt}
\tablehead{
\colhead{Source\tablenotemark{a}} &
\colhead{\gl} &
\colhead{\gb} &
\colhead{Radius} &
\colhead{$T_L$} &
\colhead{$\sigma T_L$} &
\colhead{$V_{LSR}$} &
\colhead{$\sigma V_{LSR}$} &
\colhead{$\Delta V$} &
\colhead{$\sigma \Delta V$} &
\colhead{rms}%& $
%\colhead{Note\tablenotemark{a}}
\\
\colhead{} &
\colhead{($\arcdeg$)} &
\colhead{($\arcdeg$)} &
\colhead{(arcmin.)} &
\colhead{(mK)} &
\colhead{(mK)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{(mK)}% &
%\colhead{}
}
\startdata
\input gdigs_newregionsdig2.tab
\enddata
\label{tab:new_dig}
\tablenotetext{a}{Source names for HII regions with multiple detected hydrogen RRL components are appended with ``a'' and ``b'' in order of decreasing hydrogen RRL intensity.}
\end{deluxetable*}

\subsection{Multiple-Velocity HII Regions}
Many discrete \hii\ regions have more than one measured RRL velocity.  For such a region, one velocity component presumably comes from the \hii\ region itself, and the other component(s) from diffuse ionized gas along the line of sight.  With their large beams and sensitivity to extended emission, single-dish observations are especially susceptible to detecting compact and diffuse RRL emission in the same pointing.  In the GBT \hii\ Region Discovery Survey \citep[HRDS;][]{anderson11}, for instance,  over 30\% of all detected \hii\ regions have more than one RRL velocity.  The kinematic distances %(Galactocentric or Heliocentric) 
to these regions cannot be determined, reducing their use for studies of Galactic structure and making computation of physical parameters difficult.

\citet{anderson15b} determined the correct velocity for 103 of the 117 multiple-velocity HRDS \hii\ regions using a variety of methods including new pointed RRL observations.
%, the electron temperatures, associations with molecular gas, and the velocities of any associated carbon RRLs.  
The new pointed RRL observations were off-source from the multiple-velocity HRDS \hii\ regions, and therefore sampled the diffuse ISM.  We can use GDIGS to do a similar experiment, sampling the diffuse ionized gas around multiple-velocity \hii\ regions.  

We compile a list of multiple-velocity \hii\ regions from the {\it WISE} catalog.
%, which contains the location and angular extent of each \hii\ region.  
We add the 26 multiple-velocity \hii\ regions from Tables~\ref{tab:groups}$-$\ref{tab:new} and the 6 multiple-velocity DIG locations to this list, for a total of 153 positions. 

The morphology of the \hna\ RRL emission for the discrete \hii\ region velocity should roughly match that defined in the {\it WISE} catalog, whereas the morphologies for diffuse ionized gas velocities will be more distributed.  In Figure~\ref{fig:multvel}, we show the GDIGS \hna\ emission for the two velocities detected for \hii\ region G010.331$-$00.287: 0.8\,\kms\ and 33.4\,\kms \citep{lockman89}.  The emission at the 0.8\,\kms\ velocity is diffuse and does not match the expected morphology.  The emission at the 33.4\,\kms\ velocity matches {\bf the expected \hii\ region morphology}, and we therefore treat this as the ``correct'' \hii\ region velocity.

\startlongtable
\begin{deluxetable}{lrrr}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Multiple RRL Velocity Locations \label{tab:multvel}}
\tablewidth{0pt}
\tablehead{
\colhead{Source} &
\colhead{HII Region $V_{LSR}$} &
\colhead{Other $V_{LSR}$} &
\colhead{Catalog}%& $
%\colhead{Note\tablenotemark{a}}
\\
\colhead{} &
\colhead{(\kms)} &
\colhead{(\kms)} &
\colhead{}% &
%\colhead{}
}
\startdata
\input gdigs_multvel2.tab
\enddata
\end{deluxetable}

{\bf We use GDIGS data to identify the \hii\ region velocity for 52 of 147
\hii\ regions that have multiple RRL velocities detected in previous pointed observations;} these are therefore the correct velocities and the other velocities come from the DIG or other nearby \hii\ regions.  We give the correct velocity for these 55 sources in Table~\ref{tab:multvel}, which lists the source name, the \hii\ region RRL velocity, the other RRL velocities detected along this line of sight, and the origin of the source (Known, Group, Candidate, Radio Quiet, New, or DIG).  For the DIG designation, the ``correct'' velocity is the one that best matches the emission seen in the Moment~0 maps.   
%GDIGS data is inconclusive for the remaining multiple-velocity nebulae.

\begin{figure*}
    \centering
    \includegraphics[width=3.65in]{G010_331_1.pdf}\hskip-0.3in
    \includegraphics[width=3.65in]{G010_331_2.pdf}    
    \caption{Example multiple-velocity \hii\ region analysis.  Shown are Moment~0 images for the two detected velocities for G10.331$-$0.278: 0.8\,\kms\ (left) and 33.4\,\kms\ (right) \citep{lockman89}. The 0.8\,\kms\ emission is dominated by other nearby \hii\ regions, whereas the 33.4\,\kms\ emission is centered on G10.331$-$0.278.  We conclude that the velocity of G10.331$-$0.278 is 33.4\,\kms, and the 0.8\,\kms\ component is from diffuse ionized gas. \label{fig:multvel}}
\end{figure*}

%\subsection{HII Region Distances}

%For newly-detected group \hii\ regions (Table~\ref{tab:groups}), we assign the distance to known \hii\ regions in the same complex.  These distances are frequently derived from maser parallax measurements, and therefore are more accurate than kinematic distances. % For the identified locations of diffuse RRL emission, we compute the kinematic distances, but do not resolve the KDA. 

%Need to use HIE/A...}.  For the other \hii\ regions newly detected in RRL emission (Tables~\ref{tab:candidates}$-$\ref{tab:new}) and the resolved multiple-velocity \hii\ regions, we make a kinematic distance ambiguity resolution (KDAR) using \hi\ absorption, in the same manner as \citet{anderson09a} and \citet{anderson12c}. To resolve the KDA we examine on- and off-source \hi\ spectra. As in previous work, we used an off-target location at a position as close to the source as possible so we could sample a similar column of hydrogen.  

%The difference of the on-and off-source spectra shows absorption of background 21\,cm radio continuum emission from the \hii\ region by foreground \hi. If absorption only occurs up to the \hii\ region velocity, the source should lie at the near distance. If absorption is detected between the \hii\ region velocity and the tangent point velocity, the source should lie at the far distance. If a source velocity is within 10\,\kms of the tangent point velocity, we use the tangent point distance, since absorption may not occur in this narrow velocity window. 
%, due to the non-circular 
%streaming motions and the difficulty of detecting \hi\ absorption 
%within such a narrow velocity range. 

%We assign each KDAR a quality factor based on our qualitative assessment of our confidence in the KDAR: ``A'' is very certain, ``B'' is less certain, and ``C'' means we cannot resolve the KDAR. Of the xxx multiple-velocity \hii\ regions we examine here that do not lie at the tangent point, we derive a KDAR for xxx. 
%This percentage is lower than that of the HRDS \citep[67\% if tangent-point sources are excluded;][]{anderson12c}. %In part this is because %although the average line intensity is higher than that of the HRDS, %there are a larger number of low intensity sources %(Figure~\ref{fig:height}) that do not cause \hi\ absorption. The %average distance for our sample here is $\input davg $\,kpc, %while it was 10.1\,kpc in the HRDS \citep{anderson12c}. 
%We give the results of our distance analysis in Table~\ref{tab:distances}.
%, which lists the source LSR velocity, the near, far, and tangent point kinematic distances, the KDAR, the quality factor for the KDAR, the Galactocentric radius, the heliocentric distance, the height above the plane, and the criteria used to determine the \hii\ region velocity. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%\begin{deluxetable*}{lrcccccccrrr} %\setlength{\tabcolsep}{6pt} %\tabletypesize{\footnotesize}
%\tablecaption{HII Region Distances} 
%\tablewidth{0pt} 
%\tablehead{ 
%\colhead{Name} & 
%\colhead{$V_{LSR}$} & 
%\colhead{$D_N$} & 
%\colhead{$D_F$} & 
%\colhead{$D_T$} & 
%\colhead{\rgal} & 
%\colhead{$V_{T}$} & 
%\colhead{KDAR$^{\rm a}$} & 
%\colhead{$D_\sun$} & 
%\colhead{$\sigma D_\sun$} & 
%\colhead{$z$} \\ \colhead{} & 
%\colhead{(\kms)} & 
%\colhead{(kpc)} & 
%\colhead{(kpc)} & 
%\colhead{(kpc)} & 
%\colhead{(kpc)} & 
%\colhead{(\kms)} & 
%\colhead{} & 
%\colhead{(kpc)} & 
%\colhead{(kpc)} & 
%\colhead{(pc)}} 
%\startdata 
%\input hrds_diffuse_distances.tab 
%\enddata 
%\tablenotetext{a}{Kinematic distance ambiguity resolution: ``T''=tangent point distance; ``O''=outer Galaxy source} %\tablecomments{Table~\ref{tab:distances} is available in its entirety in the electronic edition of the {\it Astrophysical Journal Supplement Series}. %A portion is shown here for guidance regarding its form and content.} 
%\label{tab:distances} 
%\end{deluxetable*} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
